Self-organized inductive reasoning with NeMuS

Neural Multi-Space (NeMuS) is a weighted multi-space representation for a portion of first-order logic designed for use with machine learning and neural network methods. It was demonstrated that it can be used to perform reasoning based on regions forming patterns of refutation and also in the process of inductive learning in ILP-like style. Initial experiments were carried out to investigate whether a self-organizing the approach is suitable to generate similar concept regions according to the attributes that form such concepts. We present the results and make an analysis of the suitability of the method in the process of inductive learning with NeMuS.

==> results.tex <==
\section{Results}\label{results}

We have presented and experimented a model for reasoning over a knowledge base using Self-Organizing Map (SOM) and one of its variants called the Associative Self-Organizing Map. The A-SOM develops a representation of its input space but also learns to associate its activity with the activities of an arbitrary number of ancillary inputs. In our experiments we connected an A-SOM to a list of main and ancillary inputs provided by the knowledge base using the NeMuS space notations. As a result, we have presented a embryonic way to induce rules using the Self-Organizing Maps.
